MLaKE: Multilingual Knowledge Editing Benchmark for Large Language Models

The extensive utilization of large language models (LLMs) underscores the crucial necessity for precise and contemporary knowledge embedded within their intrinsic parameters. Existing research on knowledge editing primarily concentrates on monolingual scenarios, neglecting the complexities presented by multilingual contexts and multi-hop reasoning. To address these challenges, our study introduces MLaKE (Multilingual Language Knowledge Editing), a novel benchmark comprising 4072 multi-hop and 5360 single-hop questions designed to evaluate the adaptability of knowledge editing methods across five languages: English, Chinese, Japanese, French, and German. MLaKE aggregates fact chains from Wikipedia across languages and utilizes LLMs to generate questions in both free-form and multiple-choice. We evaluate the multilingual knowledge editing generalization capabilities of existing methods on MLaKE. Existing knowledge editing methods demonstrate higher success rates in English samples compared to other languages. However, their generalization capabilities are limited in multi-language experiments. Notably, existing knowledge editing methods often show relatively high generalization for languages within the same language family compared to languages from different language families. These results underscore the imperative need for advancements in multilingual knowledge editing and we hope MLaKE can serve as a valuable resource for benchmarking and solution development.

==> section/related_work.tex <==
\section{Related Work}
We introduce recent datasets and knowledge editing methods in this section.

\subsection{Knowledge Editing Datasets}
\label{Knowledge Editing Dataset}
Current research in knowledge editing datasets predominantly focuses on monolingual contexts. For instance, RIPPLEEDITS~\citep{DBLP:journals/corr/abs-2307-12976}, with its 5,000 instances of factual edits in English, serves as a pivotal benchmark designed to examine the ripple effects in knowledge editing processes. Similarly, MQuAKE delves into English multi-hop queries~\citep{DBLP:journals/corr/abs-2305-14795}, evaluating how edits influence intricate chains of knowledge. KEbench offers a thorough assessment of the stability of various knowledge editing methods using a tree-structured dataset in English. In contrast, the works of Bi-ZsRE~\citep{DBLP:journals/corr/abs-2309-08952} and MzsRE~\citep{DBLP:journals/corr/abs-2312-13040} extend to a multilingual knowledge editing dataset by translating the English Zero-Shot Relation Extraction (ZsRE)~\citep{DBLP:conf/conll/LevySCZ17} dataset into various languages. Nonetheless, such endeavors in translation might introduce discrepancies in entity alignment, thereby possibly diminishing the quality of datasets ~\citep{DBLP:journals/corr/abs-2309-08952}.

\subsection{Knowledge Editing Methods}

Current knowledge editing methods can be classified into four paradigms based on knowledge storage and learning techniques: locate-then-edit, memory-based models, meta-learning, and knowledge augmentation. \textbf{Locate-Then-Edit} involves identifying and updating a subset of model parameters associated with the edited knowledge. For instance, \citet{dai-etal-2022-knowledge} manipulates `knowledge neurons' (KN) within pretrained transformers to update facts. Similarly, \citet{DBLP:conf/nips/MengBAB22} introduces a method called Rank-One Model Editing (ROME) that modifies key feedforward weights to edit factual associations in LLMs.  However, both ROME and KN are limited to modifying one piece of knowledge at a time. To address this limitation, \citet{DBLP:conf/iclr/MengSABB23} extended the capabilities of ROME and developed MEMIT, enabling batch modification of knowledge simultaneously~\citep{DBLP:journals/corr/abs-2301-04213,DBLP:journals/corr/abs-2311-09053}. \textbf{Memory-based Model} facilitates editing by introducing a small auxiliary model or additional parameters within the MLP layer, without altering the parameters of the original model. SERAC is a method that modifies knowledge by optimizing a counterfactual model~\citep{DBLP:conf/icml/MitchellLBMF22}. On the other hand, T-Patcher achieves knowledge editing by integrating a few trainable neuron patches into the MLP layer~\cite{DBLP:conf/iclr/HuangSZZR023}. In addition, CALINET leverages the characteristics of MLP layers to directly calibrate factual knowledge within LLMs~\citep{dong-etal-2022-calibrating}. \textbf{Meta-learning} utilizes a hypernetwork specifically designed to handle the necessary alterations for manipulating knowledge within the MLP layers of models. KnowledgeEditor~\citep{de-cao-etal-2021-editing} make use of hypernetworks to facilitate efficient edits in language models. MEND~\citep{DBLP:conf/iclr/MitchellLBFM22} introduces auxiliary networks and enables scalable edits by decomposing gradients. \textbf{Knowledge augmentation} mainly includes StableKE ~\citep{wei2024stable} method enhances the stability and effectiveness of knowledge editing in large language models through two automated knowledge augmentation strategies: Semantic Paraphrase Enhancement and Contextual Description Enrichment.


\begin{comment}


\end{comment}
